Co(ve)rtex: ML Models as storage channels and their (mis-)applications

Machine learning (ML) models are overparameterized to support generality and avoid overfitting. The state of these parameters is essentially a "don't-care" with respect to the primary model provided that this state does not interfere with the primary model. In both hardware and software systems, don't-care states and undefined behavior have been shown to be sources of significant vulnerabilities. In this paper, we propose a new information theoretic perspective of the problem; we consider the ML model as a storage channel with a capacity that increases with overparameterization. Specifically, we consider a sender that embeds arbitrary information in the model at training time, which can be extracted by a receiver with a black-box access to the deployed model. We derive an upper bound on the capacity of the channel based on the number of available unused parameters. We then explore black-box write and read primitives that allow the attacker to:(i) store data in an optimized way within the model by augmenting the training data at the transmitter side, and (ii) to read it by querying the model after it is deployed. We also consider a new version of the problem which takes information storage covertness into account. Specifically, to obtain storage covertness, we introduce a new constraint such that the data augmentation used for the write primitives minimizes the distribution shift with the initial (baseline task) distribution. This constraint introduces a level of "interference" with the initial task, thereby limiting the channel's effective capacity. Therefore, we develop optimizations to improve the capacity in this case, including a novel ML-specific substitution based error correction protocol. We believe that the proposed modeling of the problem offers new tools to better understand and mitigate potential vulnerabilities of ML, especially in the context of increasingly large models.

==> sections/motivation.tex <==
\section{Background and Motivation}~\label{sec:motivation}

Machine learning models are defined by a large number of parameters; in the case of neural networks these parameters represent the weights on incoming edges for neurons.  The parameters are determined through iterative training of these models using a training data set.  Specifically, a training process such as stochastic gradient descent uses backpropagation through the network to adapt the parameters to minimize a loss function, improving the accuracy of the model~\cite{ml-training}.  


\noindent 
{\bf ML models as storage channels:} Through the training process, the values of the parameters are indirectly affected by the inputs and labels of the training data.  The training process may therefore be viewed as {\em storing values} that are a function of the training data in the model parameters.  Carrying the same analogy, these {\em stored values can then be read}, either directly by someone with white-box access to the model, or indirectly by someone with access to query the model (black-box access).    

\noindent 
{\bf Unused parameters in ML models:} The size of ML models continues to increase to enhance their ability to generalize to increasingly more complex tasks, as well as to support better generalization and avoid overfitting.  The number of parameters in some models is now measured in billions~\cite{gpt3,mt-nlg} and expectedly in trillions \cite{gpt4}.  A trained model ends up using only a subset of the available parameters, leaving a large number of parameters that are not important for the performance of the baseline model~\cite{paul2022lottery}.  This gives rise to optimizations such as quantization and pruning to reduce the overhead of training and inference; these optimizations exploit the fact that there is unused capacity in the model that can be reduced without affecting the model accuracy~\cite{quantization,paul2022lottery}.  

\noindent 
{\bf \ourapproach--exploiting unused capacity as a covert storage channel:} The premise of this paper is that we can use the available unused parameters in an ML model to store information during training, creating a covert storage channel.  The channel is covert in the sense that it does not affect the performance of the baseline model, and it requires the receiver to know the addressing scheme used by the sender to be able to retrieve the stored message.  Creating such a storage channel raises a number of fundamental questions, which we discuss briefly below.  Potential applications (and exploitations!) of this channel are also discussed below.

\noindent
{\bf Encoding information in ML models:} In order to turn ML models into storage channels, we need to come up with primitives that can efficiently encode the information when it is stored and to recover it when it is to be read.    In a black box setting where the attacker reads the data by providing chosen inputs to the model, the data is encoded in the output class information for each input.  Storing information is complicated by several issues, especially under the black box model where the attacker cannot access the model parameters directly, including: (1) preserving the primary model. the stored information should not degrade the quality of the baseline/primary model; otherwise, it is easy to discern that the model has been modified and has lower accuracy; (2) Creating an address space and store/read primitives to enable storage: how can we systematically create an address space that enables us to identify where information is stored and how to recover it?  How can information be stored and retrieved?  The problem is complicated because writing of a value at an "address" has to be done through the training process, which does not provide direct control to use the available parameters; and (3) Tolerating errors in the stored data. How do we improve the quality of the channel and reduce the impact of noise?  Traditional error detection and correction can help, but we identify opportunities for error correction that leverage the properties of ML models.

\noindent 
{\bf Applications of \ourapproach:} A baseline application of \ourapproach~ is to provide a channel for communication between an entity with direct or indirect (through data) access to modify the training process, and an entity with direct or indirect (through querying the model) access to the trained model.  This channel can be used to compromise the privacy of the training data, for example: in this scenario, the attacker can encode private information about the training data in the model to allow a receiver to retrieve it by querying the model.  We believe many additional applications can arise: for example, in a federated learning setting, clients can establish covert communication channels by storing information in their models, that can be read by a colluding client in the aggregated model~\cite{federated-learning}.  In addition, this view of ML models can be used to explain and provide an alternative context to reason about a number of existing applications.  For example, backdoor attacks through data poisoning can be thought of as storing a different class value for a subset of the inputs that satisfy the trigger condition~\cite{backdoor}.  Similarly, model watermarking can be thought of as storing a watermark in the storage channel that can be recovered and verified by the receiver~\cite{deepsign}. 

%Introduce the idea of how through training a model we are actually storing values in the parameters.  If there is a primary model then the potentially available storage space is that of the extra parameters from overparameterization.  Perhaps present prior examples that have used this extra capacity.  The NDSS covert model paper; the malware hiding paper; watermarking; continual learning...


%\begin{itemize}
%    \item Discuss the tasks balance 
%    \item Correlate the over-parametrization to the capacity concept 
%    \item Show some use cases: image, text, voice, etc. 
%\end{itemize}

==> sections/sampling.tex <==
Because of the fact that the malicious model might not always have perfect accuracy for patched instances, a series of experiments are performed to ensure confidence of the readings. In such an experiment, instead of performing a single read, we perform a series of $N$ reads for each type of patched samples. As $N$ increases the probability of the correct class read being the most frequent class increases compared to the incorrect classes.

We showcase the phenomenon with a series of $N$ multinomial experiments with $K$ classes making a few minor assumptions. First, we assume that the consecutive reads are independent, which is clearly not the case. Second, we assume that the probability distribution of the incorrect classes is distributed uniformly or geometrically decreasing, however, it can be totally arbitrary. Although, the outcome is mostly affected by the next most probable class, and the effect of the other classes will be relatively insignificant.

In order to plot the behavior of the model described above, we discovered that it is difficult to derive a mathematical closed-form equation, and therefore, we veered towards a simulation-based derivation. We used Monte Carlo simulation to use randomness to our advantage to find out the required among of sample sized needed to achieve a certain amount of confidence (in this case, probability of correct read). 

In Fig. \ref{fig:uniread}, we provided the correct class with the labeled probability $P_C$ and distributed the remaining probabilities among the incorrect classes uniformly. This figure demonstrates that, for a fixed $P_C$, in order to ensure greater probability of the correct read we need larger number of reads. Also, for a smaller $P_C$, it becomes difficult to differentiate the correct class from the incorrect class by the number of observed outcomes, and therefore, a larger number of reads is required.

\begin{figure}[!th]
    \centering
    \includegraphics[width=2.5in]{figures/out1.png} 
    \caption{Probability of correct read with respect to number of reads where the probabilities of the incorrect classes are uniform}
    \label{fig:uniread}
\end{figure}

In Fig. \ref{fig:georead}, we show the effect of geometrically decreasing the probabilities of the incorrect classes, instead of distributing uniformly. As now the next most probable class has higher probability than the previous case, it becomes difficult to separate this class with the correct class. As a result, the whole plot shifts to the right, indicating larger number of required reads.  

\begin{figure}[!th]
    \centering
    \includegraphics[width=2.5in]{figures/out2.png} 
    \caption{Probability of correct read with respect to number of reads where the probabilities of the incorrect classes are geometrically decreasing}
    \label{fig:georead}
\end{figure}

Lastly, in Fig. \ref{fig:numcls} we show the effect of varying number of possible outcomes with the initial assumption that the probabilities of the incorrect classes are distributed uniformly. With fewer classes, the probabilities of the incorrect classes are larger, and as a result, an increasing number of reads are required to achieve a certain probability that the correct class is read.
\begin{figure}[!th]
    \centering
    \includegraphics[width=2.5in]{figures/out3.png} 
    \caption{Probability of the correct read when the number of classes are varied}
    \label{fig:numcls}
\end{figure}



